ELT-Bench: An End-to-End Benchmark for Evaluating AI Agents on ELT Pipelines

Practitioners are increasingly turning to Extract-Load-Transform (ELT) pipelines with the widespread adoption of cloud data warehouses. However, designing these pipelines often involves significant manual work to ensure correctness. Recent advances in AI-based methods, which have shown strong capabilities in data tasks, such as text-to-SQL, present an opportunity to alleviate manual efforts in developing ELT pipelines. Unfortunately, current benchmarks in data engineering only evaluate isolated tasks, such as using data tools and writing data transformation queries, leaving a significant gap in evaluating AI agents for generating end-to-end ELT pipelines. To fill this gap, we introduce ELT-Bench, an end-to-end benchmark designed to assess the capabilities of AI agents to build ELT pipelines. ELT-Bench consists of 100 pipelines, including 835 source tables and 203 data models across various domains. By simulating realistic scenarios involving the integration of diverse data sources and the use of popular data tools, ELT-Bench evaluates AI agents' abilities in handling complex data engineering workflows. AI agents must interact with databases and data tools, write code and SQL queries, and orchestrate every pipeline stage. We evaluate two representative code agent frameworks, Spider-Agent and SWE-Agent, using six popular Large Language Models (LLMs) on ELT-Bench. The highest-performing agent, Spider-Agent Claude-3.7-Sonnet with extended thinking, correctly generates only 3.9% of data models, with an average cost of $4.30 and 89.3 steps per pipeline. Our experimental results demonstrate the challenges of ELT-Bench and highlight the need for a more advanced AI agent to reduce manual effort in ELT workflows. Our code and data are available at https://github.com/uiuc-kang-lab/ELT-Bench.

==> content/extra/airbyte_config.tex <==
\begin{figure}[t!]

\centering

\begin{lstlisting}[frame=single]
configuration = {
  database_config = {
    self_managed_replica_set = {
      connection_string = "mongodb://elt-
        mongodb:27017/?directConnection=true"
    }
  }
}
\end{lstlisting}

\caption{A complete example of using the HuggingFace inference API in \sn.}
\label{fig:airbyte-config}

\end{figure}

==> content/extra/elt_config.tex <==
\begin{figure}[t!]

\centering

% \begin{lstlisting}[frame=single]
% mongodb:
%   config:
%     connection_string: "mongodb://elt-mongodb
%       :27017/?directConnection=true"
% \end{lstlisting}

\caption{A complete example of using the HuggingFace inference API in \sn.}
\label{fig:elt-config}

\end{figure}

==> content/extra/parameter_table.tex <==
% \begin{table}[h]
%     \centering
%     \caption{Test}
%     \label{tab:para}
%     \begin{tabular}{l|l|l}
%         \toprule
%         \textbf{Parameters} & \makecell[l]{\textbf{Spider-Agent}} & \textbf{SWE-Agent} \\
%         \midrule
%         Temperature & 0 & 0 \\

%         Top\_p & 0.9 & 1 \\

%         Max output tokens & 2500 & None\footnote{The default setting of SWE-Agent is set to None, meaning it follows the output token limit of the LLM.} \\
%         Memory length & 25 & 25 \\
%         % \midrule
%         % Step/Cost limit & 100 Steps & \makecell[l]{\$6 (GPT-4o, \\ 
%         % Claude-3.5-Sonnet) \\ 
%         % \$3 (DeepSeek-R1) \\ 
%         % \$2 (Llama-3.1-405B, Qwen\\ 2.5-Coder-32B-Instruct)} \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[h]
    \centering
    \caption{Parameter settings of Spider-Agent and SWE-Agent.}
    \label{tab:para}
    \begin{tabular}{l|l|l}
        \toprule
        \textbf{Parameters} & \textbf{Spider-Agent} & \textbf{SWE-Agent} \\
        \midrule
        Temperature & 0 & 0 \\
        Top\_p & 0.9 & 1 \\
        Max output tokens & 2500 & \makecell[l]{Same as the LLM’s\\ output token limit.} \\  
        Memory length & 25 & 25 \\
        \bottomrule
    \end{tabular}
\end{table}

==> content/limitaion.tex <==
\section{Limitaions}

==> content/old_case_study.tex <==
\section{Case Study}
\label{sec:case_study}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/case_study/4o_improved.pdf}
    \caption{Number of failed tasks by error type in Stage 1 for Spider-Agent GPT-4o and Spider-Agent-ELT GPT-4o. As shown, Spider-Agent-ELT GPT-4o reduces failures across all error categories in Stage 1.}
    \label{fig:case_study}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/results/error_bar4.pdf}
    \caption{Statistics of Spider-Agent-ELT GPT-4o in Stage 2.}
    \label{fig:case_study_stg2}
\end{figure}


Based on the error analyses in Sections~\ref{subsec:stg1_error} and \ref{subsec:stg2_error}, we improve our prompt design and introduce Spider-Agent-ELT GPT-4o. As shown in Table~\ref{tab:main_results}, Spider-Agent-ELT GPT-4o achieves a 56\% success rate in the data extraction \& loading stage, representing a 273\% improvement over Spider-Agent GPT-4o. We also compare both agents’ performances across each error type in Stage 1. As illustrated in Figure~\ref{fig:case_study}, Spider-Agent-ELT GPT-4o reduces failures in every error category in Stage 1. 

We present the performance of Spider-Agent-ELT GPT-4o in Stage 2 in Figure~\ref{fig:case_study_stg2}. Compared to Spider-Agent GPT-4o, it demonstrates better performance since more data models fail due to excessive iterations and SQL semantic errors. While the early termination issue is resolved, we observe increased semantic error types. For instance, an invalid data type issue arises when a column value is incompatible with its data type. This issue cannot be detected by DBT and requires validation within \texttt{Snowflake}, which should be considered when designing a more advanced agent to automate the ELT workflow.

==> content/old_introduction.tex <==
\section{Introduction}
% importance of ELT 
With the rise of scalable cloud-based data warehouses and the decreasing cost of storage, data engineers are increasingly using Extract-Load-Transform (ELT) pipelines to integrate data and efficiently transform it into the required format for downstream tasks \cite{seenivasan2022etl, mbata2024surveypipelinetoolsdata, FOIDL2024111855, singhal2022etl, ETLhistory}. 
For example, TPC-DI benchmark requires the creation of a decision support system for a retail brokerage firm by transforming data from various sources, including trading systems and internal Human Resources (HR) and Customer Relationship Management (CRM) systems \cite{TPCDI}. These data sources typically vary in formats, data types, attributes, and inter-table relationships \cite{TPCDI}. To build such a decision support system, data engineers can design an ELT pipeline: first, extracting and loading data into the data warehouse, followed by writing transformation queries to process and structure the data for analysis.
% , as shown in Figure~\ref{fig:elt_fig}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/elt_fig4.pdf}
%     \caption{A Complete ELT pipeline.}
%     \label{fig:elt_fig}
% \end{figure}

Compared to traditional Extract-Transform-Load (ETL) pipelines, ELT pipelines ingest data directly into data warehouses, enabling real-time Business Intelligence (BI) analysis \cite{OnDemandELT}. Furthermore, with cloud infrastructure, ELT enhances scalability for processing large volumes of data \cite{ETLhistory} and offers greater flexibility in incorporating additional data transformations \cite{ETLvsELT}. These benefits make ELT pipelines an increasingly preferred choice for processing data across various scenarios \cite{seenivasan2022etl, mbata2024surveypipelinetoolsdata, FOIDL2024111855, singhal2022etl, ETLhistory}.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/eltbench3.pdf}
    \caption{ELT-Bench is the first end-to-end benchmark designed to evaluate ability of AI agent to build ELT pipelines. The agent must construct complete ELT pipelines from scratch by decomposing the complex workflow, interacting with databases and data tools, and writing code and SQL queries.}
    \label{fig:eltbench}
\end{figure*}

% In contrast to traditional Extract-Transform-Load (ETL) pipelines, Extract-Load-Transform (ELT)  pipelines ingest data directly into data warehouses, thereby satisfying real-time Business Intelligence (BI) requirements \cite{OnDemandELT}. They also leverage cloud infrastructure to enhance scalability for processing large volumes of data \cite{ETLhistory} and offer greater flexibility in incorporating additional data transformations \cite{ETLvsELT}. Therefore, with the rise of scalable cloud-based data warehouses and the decreasing cost of storage, data engineers are increasingly adopting ELT pipelines to integrate data from multiple data sources and then convert it into a usable, reliable format for data science and Artificial Intelligence (AI) projects \cite{seenivasan2022etl, mbata2024surveypipelinetoolsdata, FOIDL2024111855, singhal2022etl}. For example, TPC-DI benchmark requires the creation of a decision support system for a retail brokerage firm by transforming data from various sources, including trading systems and internal Human Resources (HR) and Customer Relationship Management (CRM) systems \cite{TPCDI}. These data sources typically vary in formats, data types, attributes, and inter-table relationships \cite{TPCDI}. To build such a decision support system, data engineers can design an ELT pipeline: first, extracting and loading data into the data warehouse, followed by writing transformation queries to process and structure the data for analysis.

% to train a random forest regression model that forecasts each customer's total spending, the data engineer may need to build an ELT pipeline that extracts data from \texttt{Amazon S3}, loads it into a database, and executes SQL transformations to generate the final feature tables \cite{eltusecase}.

% As the volume of data and the variety of data sources continue to grow, data engineers are increasingly building ELT (Extract, Load, Transform) pipelines to convert raw data into a usable and reliable format for data science and artificial intelligence projects \cite{etl}. Consequently, the global data pipeline tools market is estimated to reach 12.09 billion dollars in 2024, with ETL data pipelines contributing the largest revenue share of 39.46\%, and is projected to grow at a compound annual growth rate (CAGR) of 26.8\% from 2025 to 2030 \cite{datamarket}. More recently, with the advent of scalable cloud-based data warehouses, the market is shifting from ETL pipelines towards ELT (Extract, Load, Transform) pipelines.

% , where data transformation occurs after the loading stage, have gained popularity. \yuxuan{This sentence basically repeats the first one. This paragraph needs re-work.}

% leveraging collected data for analytics, data science, and machine learning initiatives to drive business insights \cite{etl}. However, raw and messy data significantly complicate downstream usage. To convert this data into a usable and reliable format, data engineers must build ETL (Extract, Transform, Load) pipeline, which extract data from multiple sources, apply transformations, and load it into a data warehouse. More recently, with the advent of scalable cloud-based data warehouses, ELT (Extract, Load, Transform) pipeline, where data transformation occurs after the loading stage, have gained popularity.
% The ELT pipeline improves the flexibility to implement new business transformations and scales effortlessly to handle larger data volumes.
% difficulty of building ELT

Developing ELT pipelines is an essential task for data engineers \cite{seenivasan2022etl, singhal2022etl, mbata2024surveypipelinetoolsdata, FOIDL2024111855, ETLhistory}, but the process requires significant manual work. First, these pipelines must extract and integrate data from disparate sources with varying formats and standards. Second, data engineers or data analysts need a deep understanding of the source data schema to write transformation queries. For example, it is estimated that over 60\% of the time in a data warehousing project is spent on building data pipelines \cite{effortestimation, datawarehouse, Researchdatawarehouse, realworlddata, Datamanipulation}.

% the process of turning raw data into a usable dataset can take about 80\% of the time in a data science project \cite{Exploratorydm}. 
% \yuxuan{Can we have more citations and one more example?}

% For instance, e-commerce businesses often seek insights into user behavior, such as preferences and average order value, to adjust sales strategies \cite{eltexamples}. To achieve this, data engineers must extract user data from various sources, including APIs, customer relationship management (CRM) systems, and relational databases, before loading it into a data warehouse. Once the data is integrated, they need to analyze the source data schemas and write complex nested queries to produce the required data models, facilitating downstream analysis.

% LLM ability
Can AI agents be used to automate the development of ELT pipelines? 
Recent advancements in Large Language Models (LLMs) have demonstrated strong capabilities in the text-to-SQL task, a crucial component of ELT pipelines. Notably, state-of-the-art (SOTA) techniques based on LLMs have achieved execution accuracy rates of 75.6\% and 91.2\% on the \bird \cite{bird} and Spider 1.0 \cite{spider1} benchmarks, respectively.
More recently, researchers have developed AI agents to tackle more complex real-world tasks that demand skills such as reasoning, tool usage, planning, and memorization \cite{ReAct, Reflexion, sweagent, spider2, codeact, weng2023agent}. 
To evaluate the capability of emerging AI agents, researchers have proposed numerous benchmarks in the data domain \cite{ds1000, dacode, InfiAgent, spider2v, spider2}. However, there is no end-to-end benchmark designed with end-to-end ELT pipelines.

% Existing benchmarks in the data domain focus on various tasks, such as data science code generation \cite{ds1000, dacode}, data analysis \cite{InfiAgent}, data application usage \cite{spider2v}, and text-to-SQL generation \cite{spider2}. 

% These benchmarks various fields, including software engineering \cite{swebench}, machine learning \cite{MLAgentBench}, and web-based interactions \cite{WebArena, WorkArena}.

% To evaluate the capabilities of LLM-powered agents, numerous benchmarks have been introduced over the years. Existing benchmarks in the data domain focus on various tasks, such as data science code generation \cite{ds1000, dacode}, data analysis \cite{InfiAgent}, data application usage \cite{spider2v}, and text-to-SQL generation \cite{spider2}. However, benchmarks within the data engineering domain are often limited to narrower tasks. For instance, Spider2-V evaluates an agent's ability to interact with different data applications, each associated with specific task descriptions \cite{spider2v}, while Spider 2.0 focuses on assessing an agent's ability to write transformation queries within existing project codebases and databases \cite{spider2}. This leaves a significant gap: the lack of an end-to-end benchmark designed to evaluate the ability of LLM-based agents to build comprehensive ELT pipelines.
Building an end-to-end ELT benchmark is challenging because it requires sophisticated setup and configuration, time-consuming ground-truth labeling, and thorough workflow verification, to ensure reproducibility and correctness. First, it is necessary to set up a variety of data management systems and platforms to store the source data and prepare the necessary data tools to ensure they can handle all relevant data sources. Second, annotators must manually annotate configuration information and clearly define target data models given input files within the project base. 
% These data models, which reflect real-world use cases in data science and AI projects, are generally not publicly available due to privacy constraints and, thus, must be manually constructed. 
Third, to evaluate the performance of an agent, annotators must label the ground truth by writing configuration files and complex transformation queries that involve multiple relational operations, including casting, converting, joining, aggregating, and ranking. Finally, annotators must run each ELT pipeline manually to confirm both the correctness of the environment and the validity of the annotations. 
% After verifying the annotated pipeline, annotators must save the source table sizes and the results of the generated data model to files for ELT-Bench evaluation.

We address these challenges by introducing ELT-Bench, a new benchmark of 100 ELT pipelines associated with 835 source tables and 203 data models across various domains. For a single ELT pipeline, we spend 3 to 5 hours of manual effort to set up the environment, annotate input files and the ground truth, and build the entire pipeline for verification. Notably, 60\% of the pipelines require extracting and integrating data from five distinct categories of sources (APIs, cloud services, relational databases, NoSQL databases, and flat files). In addition, the ground truth for each pipeline, on average, involves 187 lines of code per configuration file and 200 SQL tokens (tokenized by whitespace \cite{spider2}) per data model.

% To address this gap, we propose a new benchmark, ELT-Bench, designed to emulate real-world, end-to-end ELT pipelines. This benchmark consists of 100 databases associated with 840 data sources and 206 data models spanning a wide range of domains, aiming to facilitate the development of advanced agents capable of automating the process of building ELT pipelines. As illustrated in Figure \ref{fig:eltbench}, our benchmark includes five types of data sources: relational databases (\texttt{PostgreSQL}), NoSQL databases (\texttt{MongoDB}), API sources, flatten files (\texttt{CSV}, \texttt{JSONL}, \texttt{Parquet}), and cloud storage files (\texttt{Amazon S3}). After extracting and loading data into the data warehouse, the agent is tasked with performing transformations such as casting, converting, joining, and aggregating raw data using SQL to generate high-quality data suitable for downstream use.

% \yuxuan{We should that we build a benchmark called ELT-Bench and then discuss details about ELT-Bench.} 
ELT-Bench is the first benchmark that covers the entire workflow for building ELT pipelines, providing a comprehensive evaluation through several interconnected subtasks. As shown in Figure \ref{fig:eltbench}, ELT-Bench requires agents to construct an end-to-end ELT pipeline from scratch, encompassing two primary stages: (1) data extraction \& loading and (2) data transformation. Agents perform actions in a sandbox environment that provides a pre-established project base. This setup replicates the real-world workflow of a data engineer, challenging AI agents to break down the complex workflow into manageable subtasks, interact with databases and data tools, write code, orchestrate every stage of the ELT pipeline, and finally generate the required data models.



% In  The interconnected subtasks setting requires revisit and refine previous steps

% ELT-Bench is first benchmark specialized for evaluating agent ability on building ELT workflow and presents a more comprehensive benchmark as it comprises several interconnected subtasks. Previous benchmarks focus on a narrower task within the data engineering domains that be a subtask of ELT-bench. For instance, Spider-2 includes examples evaluating the ability of agent to write tranformation queries with existing project codebases and databases \cite{spider2}. Instead, ELT-Bench challenges agents to construct an end-to-end ELT workflow from scratch, encompassing two primary stages: (1) data extraction and loading, and (2) data transformation. The agent begins in a sandbox environment, equipped with provided files containing nessacary configurations to access data sources, destinations, and applications, as well as schemas of data sources and the specifications for desired data models. This setting simulates real-world data engineer work, requiring agent to decompose the complex task into subtasks and go back to a previous subtasks and refine, interact with both databases and data applications (tool usage), writing code, and finally generate the desired data models. The agent are required to simulate human actions to interact with the environment, including writing code, using data applications, addressing feedback from the environment, and ultimately generating the required data models. This comprehensive design ensures that ELT-Bench effectively evaluates an agent's ability (reasoning, planning, memorization and tool usage) to handle the complexity of real-world, end-to-end data engineering workflows.

We evaluate two code agent frameworks, Spider-Agent \cite{spider2} and SWE-Agent \cite{sweagent}, with popular LLMs on ELT-Bench. The top-performing agent, Spider-Agent Claude-3.7-Sonnet with extended thinking, achieves a success rate of 57\% in the data extraction \& loading stage but only a success rate of 3.9\% in the data transformation stage. On average, Spider-Agent Claude-3.7-Sonnet consumes \$4.30 and requires 89.3 execution steps per task (under a 100-step limit). The poor performance and relatively high operational cost highlight the need for further advancements in AI agents to facilitate automated ELT workflows.

% We evaluated two code generation agent frameworks—Spider-Agent [29] and SWE-Agent [30]—in combination with five popular LLMs on ELT-Bench. The top-performing agent, SWE-Agent Claude, achieves a 37% success rate in extracting and loading data, but only 1% in data model generation. Building on these findings, we enhanced Spider-Agent GPT-4o to form Spider-Agent-ELT GPT-4o, which attains a 56% success rate for extracting and loading data and a 0.5% success rate for data model generation. These results underscore the need for more advanced agents and further research to support automated ELT workflows.

% In summary, our contributions are as follows:
% \begin{enumerate}[leftmargin=1.5em, topsep=0.1em]
%   \item We propose ELT-Bench, a benchmark for evaluating the ability of AI agents to construct end-to-end ELT pipelines. 

%   \item We evaluate two code generation frameworks with five popular LLMs. 

% \end{enumerate}
% 3. 开头和第二段衔接， 再引出llm 把第三段拆成两个自然段：agent work， benchmark work，删除第五段detail

==> figures/case_study/prompt.tex <==
\begin{tcolorbox}[
    colback=red!5!white,     % Background color
    colframe=red!50!black,   % Border color
    title=Failure case,
    fonttitle=\bfseries,       % Title font style
    arc=2mm,                   % Rounded corners
    boxrule=1pt,               % Border thickness
    top=1mm, bottom=1mm,
    left=1mm, right=1mm
]
\medskip
\textbf{Action 1:} Bash(code="cat /workspace/config.yaml")  \\
\textbf{Action 6:} EditFile(filepath="/workspace/elt/main.tf")
\small
\begin{verbatim} 
```resource "airbyte_destination" "snowflake" {
password  = "Snowflake@123"}
 (Omitted other fields)
```
\end{verbatim} 
\normalsize
\textbf{Action 8:} Bash(code="terraform apply -auto-approve") \\
\textbf{Observation-8:} The provider airbytehq/airbyte does not support resource type "airbyte\_destination"\\
\textbf{Action 14:}Bash(code="cat /workspace/documentation/destination\_snowflake.md")
\small
\begin{verbatim} 
```
resource "airbyte_destination_snowflake"    "snowflake"{
    password  = "Snowflake@123"}
(Omitted other fields)
```
\end{verbatim} 
\normalsize
...
\end{tcolorbox}

==> figures/example/incorrect_source_type.tex <==
\begin{figure}[t]
  \begin{subfigure}[t]{\columnwidth}
    \begin{lstlisting}[style=terraform]
resource "airbyte_destination" "my_destination"
\end{lstlisting}
\caption{Incorrect resource type.}
\label{sub:iccor_resource}
\end{subfigure}

 \vspace{1em}

  \begin{subfigure}[t]{\columnwidth}
    \begin{lstlisting}[style=terraform]
resource "airbyte_destination_snowflake" "my_destination"
\end{lstlisting}
\caption{Correct resource type.}
\label{sub:cor_resource}
\end{subfigure}

\caption{Correct and incorrect code examples for configuring the \texttt{Snowflake} destination resource type in \texttt{Airbyte}.}
\label{fig:resourece}
\end{figure}


==> figures/example/snowflake.tex <==
\begin{figure}[t]
    \begin{lstlisting}[style=terraform]
credentials = {
      username_and_password = {
        password = "<password>"
      }
    }
\end{lstlisting}

\caption{The correct format to write the \texttt{Snowflake} password field.}
\label{fig:cor_sf}
\end{figure}

==> tables/stage_1.tex <==
\begin{table}[h]
    \centering
    \caption{Stage 1 Common Error.}
    \label{tab:stg1_results}
\begin{tabular}{l c r r r r}
\toprule
\textbf{} & \textbf{Spider-Agent} & \textbf{SWE-Agent} & \textbf{SRDM (\%) } & \textbf{Average Cost (\$)} & \textbf{Average Steps} \\
\midrule
 & GPT-4o & 15\% & 0 & 2.4 & 44.1 \\
 & Claude-3.5-Sonnet & 0 & 0.5\% & 3.7 & 65.9 \\
\midrule
 & GPT-4o & 0 & 0 & 2.3 & 61.2 \\
 & Claude-3.5-Sonnet & 37\% & 1\% & 5.2 & 60 \\
\bottomrule
\end{tabular}

\end{table}
